Comparing methods addressing multi-collinearity when developing prediction models

Clinical prediction models are developed widely across medical disciplines. When predictors in such models are highly collinear, unexpected or spurious predictor-outcome associations may occur, thereby potentially reducing face-validity and explainability of the prediction model. Collinearity can be dealt with by exclusion of collinear predictors, but when there is no a priori motivation (besides collinearity) to include or exclude specific predictors, such an approach is arbitrary and possibly inappropriate. We compare different methods to address collinearity, including shrinkage, dimensionality reduction, and constrained optimization. The effectiveness of these methods is illustrated via simulations. In the conducted simulations, no effect of collinearity was observed on predictive outcomes. However, a negative effect of collinearity on the stability of predictor selection was found, affecting all compared methods, but in particular methods that perform strong predictor selection (e.g., Lasso).}

==> sections/3-TABS-COEFF.tex <==
% \newtoggle{inTableHeader}% Track if still in header of table
% \toggletrue{inTableHeader}% Set initial value
% \newcommand*{\StartTableHeader}{\global\toggletrue{inTableHeader}}%
% \newcommand*{\EndTableHeader}{\global\togglefalse{inTableHeader}}%




% % Redefine tabular to initialize \StartTableHeader at start and end
% \let\OldTabular\tabular%
% \let\OldEndTabular\endtabular%
% \renewenvironment{tabular}{\StartTableHeader\OldTabular}{\OldEndTabular\StartTableHeader}%
 
 %The min, mid and max values
\newcommand*{\MinCoefNumber}{-2.0}%
\newcommand*{\MidCoefNumber}{0.0} %
\newcommand*{\MaxCoefNumber}{1}%


\newcommand*{\MinCoefColor}{cyan}%
\newcommand*{\MidCoefColor}{white} %
\newcommand*{\MaxCoefColor}{red}%

%Apply the gradient macro
\newcommand{\ApplyCoefGradient}[1]{%
  \iftoggle{inTableHeader}{#1}{
    \ifdim #1 pt > \MidCoefNumber pt
        \pgfmathsetmacro{\PercentColor}{max(min(100.0*(#1 - \MidCoefNumber)/(\MaxCoefNumber-\MidCoefNumber),100.0),0.00)} %
        \hspace{-0.33em}\colorbox{\MaxCoefColor!\PercentColor!\MidCoefColor}{\hspace{3pt}#1\hspace{0pt}}
    \else
        \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MidCoefNumber - #1)/(\MidCoefNumber-\MinCoefNumber),100.0),0.00)} %
        \hspace{-0.33em}\colorbox{\MinCoefColor!\PercentColor!\MidCoefColor}{#1}
    \fi
  }}

\newcolumntype{R}{>{\collectcell\ApplyCoefGradient}l<{\endcollectcell}}
\renewcommand{\arraystretch}{0}
%\setlength{\fboxsep}{1mm} % box size
\setlength{\tabcolsep}{2pt}


\begin{table}[h!]
    \caption{\label{tab:coef:xerbasic}Model coefficients for \xerbasic}
\resizebox{\textwidth}{!}{
\begin{tabular}{lRlRlRlRlRlRlRlRlRlRlRlRlRlRlRlRlR}\toprule 
 &\multicolumn{2}{l}{\textbf{LR}}&\multicolumn{2}{l}{\textbf{Lasso}}&\multicolumn{2}{l}{\textbf{Ridge}}&\multicolumn{2}{l}{\textbf{ElasticNet}}&\multicolumn{2}{l}{\textbf{PCLR}}&\multicolumn{2}{l}{\textbf{LAELR}}&\multicolumn{2}{l}{\textbf{Dropout}}&\multicolumn{2}{l}{\textbf{\LRnn{}}}\\\midrule
\textbf{Summary} \\
\sumNegOarCoef{}&-0.08&$^{(-0.59, 0.00)}$&0.00&$^{(-0.39, 0.00)}$&0.00&$^{(-0.34, 0.00)}$&0.00&$^{(-0.19, 0.00)}$&0.00&$^{(-0.34, 0.00)}$&0.00&$^{(-0.60, 0.00)}$&0.00&$^{(0.00, 0.00)}$&0.00&$^{(0.00, 0.00)}$\\
\sumPosOarCoef{}&1.77&$^{(1.45, 2.39)}$&1.34&$^{(1.32, 2.18)}$&1.34&$^{(1.21, 2.10)}$&1.33&$^{(1.19, 2.02)}$&1.72&$^{(1.45, 2.13)}$&1.70&$^{(1.46, 2.39)}$&1.27&$^{(1.10, 2.03)}$&1.71&$^{(1.45, 2.36)}$\\
\percNegOarCoef{}&0.25&$^{(0.00, 0.25)}$&0.00&$^{(0.00, 0.25)}$&0.00&$^{(0.00, 0.25)}$&0.00&$^{(0.00, 0.25)}$&0.00&$^{(0.00, 0.25)}$&0.00&$^{(0.00, 0.25)}$&0.00&$^{(0.00, 0.00)}$&0.00&$^{(0.00, 0.00)}$\\
\percPosOarCoef{}&0.75&$^{(0.75, 1.00)}$&1.00&$^{(0.75, 1.00)}$&1.00&$^{(0.75, 1.00)}$&1.00&$^{(0.75, 1.00)}$&1.00&$^{(0.75, 1.00)}$&1.00&$^{(0.75, 1.00)}$&1.00&$^{(0.75, 1.00)}$&0.75&$^{(0.75, 1.00)}$\EndTableHeader\\\grayline
\textbf{Complete}\\
Intercept&-1.51&$^{(-1.80, -1.24)}$&-1.33&$^{(-1.72, -1.20)}$&-1.34&$^{(-1.67, -1.14)}$&-1.33&$^{(-1.63, -1.21)}$&-1.52&$^{(-1.67, -1.24)}$&-1.53&$^{(-1.81, -0.65)}$&-1.29&$^{(-1.62, -1.14)}$&-1.52&$^{(-1.79, -1.24)}$\\
Age&-0.02&$^{(-0.22, 0.23)}$&-0.02&$^{(-0.18, 0.18)}$&-0.04&$^{(-0.19, 0.18)}$&-0.01&$^{(-0.18, 0.15)}$&-0.02&$^{(-0.22, 0.18)}$&-0.02&$^{(-0.21, 0.23)}$&-0.03&$^{(-0.16, 0.16)}$&-0.02&$^{(-0.22, 0.23)}$\\
Xer.BSL.1&0.34&$^{(0.12, 0.49)}$&0.24&$^{(0.05, 0.45)}$&0.26&$^{(0.11, 0.45)}$&0.25&$^{(0.07, 0.44)}$&0.31&$^{(0.13, 0.49)}$&0.31&$^{(0.09, 0.46)}$&0.12&$^{(0.11, 0.41)}$&0.33&$^{(0.12, 0.49)}$\\
Xer.BSL.2&0.16&$^{(-0.27, 4.41)}$&0.04&$^{(-0.01, 0.26)}$&0.10&$^{(-0.05, 0.30)}$&0.07&$^{(-0.01, 0.24)}$&0.15&$^{(-0.21, 1.19)}$&0.16&$^{(-0.21, 14.67)}$&0.08&$^{(-0.18, 1.90)}$&0.16&$^{(-0.29, 3.81)}$\\
\grayline
Subm.L.Dm&-0.08&$^{(-0.59, 0.32)}$&0.01&$^{(-0.39, 0.30)}$&0.20&$^{(-0.34, 0.35)}$&0.11&$^{(-0.19, 0.34)}$&0.45&$^{(-0.34, 0.57)}$&0.45&$^{(-0.60, 0.50)}$&0.33&$^{(-0.01, 0.38)}$&0.00&$^{(0.00, 0.32)}$\\
Subm.R.Dm&0.85&$^{(0.43, 1.47)}$&0.49&$^{(0.33, 1.30)}$&0.37&$^{(0.30, 1.02)}$&0.41&$^{(0.29, 1.06)}$&0.44&$^{(0.29, 1.05)}$&0.44&$^{(0.30, 1.47)}$&0.39&$^{(0.31, 0.83)}$&0.80&$^{(0.43, 1.46)}$\\
Parotid.L.Dm&0.58&$^{(0.18, 0.89)}$&0.46&$^{(0.17, 0.79)}$&0.37&$^{(0.18, 0.78)}$&0.40&$^{(0.18, 0.73)}$&0.43&$^{(0.15, 0.87)}$&0.42&$^{(0.21, 0.89)}$&0.31&$^{(0.22, 0.65)}$&0.54&$^{(0.18, 0.77)}$\\
Parotid.R.Dm&0.34&$^{(0.06, 0.64)}$&0.37&$^{(0.10, 0.69)}$&0.41&$^{(0.14, 0.68)}$&0.41&$^{(0.16, 0.70)}$&0.40&$^{(0.06, 0.88)}$&0.39&$^{(0.12, 0.86)}$&0.25&$^{(0.20, 0.55)}$&0.36&$^{(0.13, 0.73)}$\\
\bottomrule
\end{tabular}}
\end{table}


\begin{table}[h!]
    \caption{\label{tab:coef:xerext}Model coefficients for \xerextended}
\resizebox{\textwidth}{!}{
\begin{tabular}{lRlRlRlRlRlRlRlRlRlRlRlRlRlRlRlRlR}\toprule 
 &\multicolumn{2}{l}{\textbf{LR}}&\multicolumn{2}{l}{\textbf{Lasso}}&\multicolumn{2}{l}{\textbf{Ridge}}&\multicolumn{2}{l}{\textbf{ElasticNet}}&\multicolumn{2}{l}{\textbf{PCLR}}&\multicolumn{2}{l}{\textbf{LAELR}}&\multicolumn{2}{l}{\textbf{Dropout}}&\multicolumn{2}{l}{\textbf{\LRnn{}}}\\
 \textbf{Summary}\\
\sumNegOarCoef{}&-3.49&$^{(-8.82, -2.12)}$&0.00&$^{(-3.51, 0.00)}$&0.00&$^{(-2.95, 0.00)}$&0.00&$^{(-2.59, 0.00)}$&0.00&$^{(-12.84, 0.00)}$&0.00&$^{(-8.67, 0.00)}$&-0.05&$^{(-0.81, 0.00)}$&0.00&$^{(0.00, 0.00)}$\\
\sumPosOarCoef{}&5.34&$^{(4.81, 12.97)}$&1.39&$^{(1.22, 6.84)}$&1.52&$^{(1.46, 6.02)}$&1.52&$^{(1.37, 4.88)}$&2.08&$^{(1.73, 17.44)}$&2.04&$^{(1.72, 13.37)}$&1.76&$^{(1.49, 2.80)}$&2.11&$^{(1.73, 5.50)}$\\
\percNegOarCoef{}&0.50&$^{(0.38, 0.62)}$&0.00&$^{(0.00, 0.38)}$&0.00&$^{(0.00, 0.50)}$&0.00&$^{(0.00, 0.50)}$&0.00&$^{(0.00, 0.50)}$&0.00&$^{(0.00, 0.56)}$&0.12&$^{(0.00, 0.25)}$&0.00&$^{(0.00, 0.00)}$\\
\percPosOarCoef{}&0.50&$^{(0.31, 0.62)}$&0.69&$^{(0.31, 0.81)}$&1.00&$^{(0.44, 1.00)}$&0.88&$^{(0.38, 1.00)}$&1.00&$^{(0.50, 1.00)}$&1.00&$^{(0.38, 1.00)}$&0.88&$^{(0.75, 1.00)}$&0.69&$^{(0.25, 0.69)}$\\\EndTableHeader\\\grayline
 \textbf{Complete}\\
Intercept&-1.75&$^{(-3.08, -1.34)}$&-1.37&$^{(-2.54, -1.17)}$&-1.40&$^{(-2.40, -1.22)}$&-1.41&$^{(-2.22, -1.20)}$&-1.66&$^{(-3.36, -1.35)}$&-1.66&$^{(-3.10, -1.35)}$&-1.47&$^{(-1.72, -1.24)}$&-1.72&$^{(-3.35, -1.35)}$\\
Age&-0.05&$^{(-0.28, 0.22)}$&-0.01&$^{(-0.14, 0.14)}$&-0.03&$^{(-0.19, 0.17)}$&-0.02&$^{(-0.20, 0.18)}$&0.04&$^{(-0.22, 0.20)}$&0.04&$^{(-0.27, 0.19)}$&-0.03&$^{(-0.12, 0.10)}$&-0.04&$^{(-0.24, 0.22)}$\\
Xer.BSL.1&0.36&$^{(0.16, 0.53)}$&0.24&$^{(0.14, 0.48)}$&0.20&$^{(0.12, 0.48)}$&0.23&$^{(0.13, 0.47)}$&0.14&$^{(0.04, 0.47)}$&0.14&$^{(-0.02, 0.53)}$&0.20&$^{(0.04, 0.35)}$&0.34&$^{(0.13, 0.51)}$\\
Xer.BSL.2&0.18&$^{(-0.24, 4.41)}$&0.05&$^{(-0.01, 0.23)}$&0.08&$^{(-0.01, 0.32)}$&0.08&$^{(-0.01, 0.31)}$&-0.12&$^{(-2.89, 4.62)}$&-0.12&$^{(-0.27, 2.00)}$&0.09&$^{(-0.16, 1.84)}$&0.19&$^{(-0.24, 3.24)}$\\
\grayline
Subm.L.Dm&-0.30&$^{(-1.46, 0.62)}$&0.04&$^{(-0.80, 0.16)}$&0.06&$^{(-0.71, 0.16)}$&0.03&$^{(-0.60, 0.16)}$&0.15&$^{(-1.07, 0.76)}$&0.15&$^{(-1.07, 0.56)}$&0.12&$^{(-0.40, 0.19)}$&0.00&$^{(0.00, 0.13)}$\\
Subm.L.V10&0.60&$^{(-0.97, 3.96)}$&0.01&$^{(-0.01, 2.41)}$&0.08&$^{(-0.38, 1.51)}$&0.07&$^{(-0.38, 1.26)}$&0.17&$^{(-1.50, 7.41)}$&0.17&$^{(-0.39, 5.36)}$&0.14&$^{(-0.02, 0.37)}$&0.02&$^{(0.00, 1.74)}$\\
Subm.L.V30&-0.72&$^{(-2.14, 0.26)}$&-0.00&$^{(-1.24, 0.02)}$&0.02&$^{(-1.10, 0.11)}$&0.00&$^{(-0.68, 0.10)}$&0.16&$^{(-4.23, 0.36)}$&0.16&$^{(-3.00, 0.35)}$&-0.01&$^{(-0.48, 0.16)}$&0.00&$^{(0.00, 0.00)}$\\
Subm.L.V50&0.39&$^{(0.02, 1.06)}$&0.05&$^{(-0.00, 0.51)}$&0.08&$^{(-0.00, 0.47)}$&0.07&$^{(-0.00, 0.35)}$&0.13&$^{(-0.15, 0.57)}$&0.13&$^{(-0.03, 0.58)}$&0.07&$^{(-0.07, 0.27)}$&0.05&$^{(0.00, 0.38)}$\\
\grayline
Subm.R.Dm&0.24&$^{(-0.64, 2.01)}$&0.15&$^{(-0.00, 1.20)}$&0.12&$^{(-0.02, 1.12)}$&0.13&$^{(-0.00, 1.25)}$&0.17&$^{(0.11, 1.15)}$&0.17&$^{(-0.52, 1.30)}$&0.16&$^{(0.03, 0.73)}$&0.16&$^{(0.00, 1.31)}$\\
Subm.R.V10&-0.05&$^{(-1.23, 1.34)}$&0.02&$^{(-0.01, 0.40)}$&0.09&$^{(0.05, 0.42)}$&0.08&$^{(-0.00, 0.36)}$&0.17&$^{(-4.14, 0.59)}$&0.17&$^{(-1.34, 0.89)}$&0.15&$^{(0.07, 0.32)}$&0.21&$^{(0.00, 0.59)}$\\
Subm.R.V30&0.55&$^{(-0.58, 2.25)}$&0.05&$^{(0.00, 1.35)}$&0.10&$^{(0.05, 0.84)}$&0.11&$^{(0.00, 0.75)}$&0.17&$^{(-0.60, 4.54)}$&0.17&$^{(-0.42, 2.26)}$&0.18&$^{(-0.02, 0.51)}$&0.47&$^{(0.00, 3.64)}$\\
Subm.R.V50&0.08&$^{(-0.72, 0.68)}$&0.16&$^{(-0.00, 0.67)}$&0.13&$^{(-0.45, 0.64)}$&0.15&$^{(-0.51, 0.62)}$&0.15&$^{(-0.46, 0.62)}$&0.14&$^{(-0.29, 0.71)}$&0.18&$^{(-0.02, 0.23)}$&0.16&$^{(0.00, 0.48)}$\\
\grayline
Parotid.L.Dm&1.36&$^{(-0.80, 4.07)}$&0.16&$^{(-0.00, 1.96)}$&0.11&$^{(0.06, 1.57)}$&0.12&$^{(-0.00, 0.88)}$&0.10&$^{(-0.01, 2.87)}$&0.13&$^{(-0.09, 3.43)}$&0.10&$^{(0.02, 0.24)}$&0.20&$^{(0.00, 0.74)}$\\
Parotid.L.V10&-0.36&$^{(-1.49, 0.57)}$&0.02&$^{(-0.69, 0.32)}$&0.12&$^{(-0.64, 0.20)}$&0.13&$^{(-0.30, 0.22)}$&0.13&$^{(-0.93, 0.28)}$&0.12&$^{(-1.22, 0.40)}$&0.13&$^{(-0.34, 0.19)}$&0.01&$^{(0.00, 0.35)}$\\
Parotid.L.V30&0.04&$^{(-1.20, 0.77)}$&0.14&$^{(-0.00, 0.53)}$&0.11&$^{(0.01, 0.39)}$&0.12&$^{(-0.01, 0.57)}$&0.09&$^{(0.03, 0.63)}$&0.08&$^{(-0.76, 0.71)}$&0.13&$^{(0.01, 0.30)}$&0.17&$^{(0.00, 0.48)}$\\
Parotid.L.V50&-0.54&$^{(-1.69, 0.36)}$&0.01&$^{(-0.80, 0.23)}$&0.05&$^{(-0.71, 0.23)}$&0.02&$^{(-0.32, 0.23)}$&0.04&$^{(-1.17, 0.27)}$&0.02&$^{(-1.27, 0.25)}$&-0.04&$^{(-0.08, 0.18)}$&0.00&$^{(0.00, 0.28)}$\\
\grayline
Parotid.R.Dm&2.09&$^{(-0.53, 3.03)}$&0.01&$^{(-0.00, 0.56)}$&0.13&$^{(0.09, 0.76)}$&0.14&$^{(0.01, 0.82)}$&0.12&$^{(0.06, 1.45)}$&0.10&$^{(0.04, 2.00)}$&0.11&$^{(-0.01, 0.21)}$&0.00&$^{(0.00, 0.42)}$\\
Parotid.R.V10&-0.25&$^{(-1.34, 0.95)}$&0.45&$^{(-0.20, 0.71)}$&0.17&$^{(-0.24, 0.56)}$&0.20&$^{(-0.13, 0.66)}$&0.14&$^{(-0.49, 0.86)}$&0.14&$^{(-0.68, 0.52)}$&0.12&$^{(0.07, 0.53)}$&0.51&$^{(0.00, 0.80)}$\\
Parotid.R.V30&-0.47&$^{(-1.00, 0.91)}$&0.15&$^{(0.00, 0.67)}$&0.13&$^{(-0.02, 0.39)}$&0.15&$^{(-0.00, 0.43)}$&0.11&$^{(-0.02, 0.52)}$&0.11&$^{(-0.47, 0.51)}$&0.13&$^{(0.05, 0.33)}$&0.17&$^{(0.00, 0.30)}$\\
Parotid.R.V50&-0.80&$^{(-1.22, 0.14)}$&-0.01&$^{(-0.48, 0.02)}$&0.04&$^{(-0.53, 0.13)}$&0.01&$^{(-0.50, 0.11)}$&0.07&$^{(-0.78, 0.17)}$&0.08&$^{(-0.92, 0.15)}$&0.03&$^{(-0.15, 0.14)}$&0.00&$^{(0.00, 0.12)}$\\
\bottomrule
\end{tabular}}
\end{table}

\newpage
\clearpage

\begin{table}[h!]
    \caption{\label{tab:coef:dysbasic}Model coefficients for \dysbasic}
\resizebox{\textwidth}{!}{
\begin{tabular}{lRlRlRlRlRlRlRlRlRlRlRlRlRlRlRlRlR}\toprule 
 &\multicolumn{2}{l}{LR}&\multicolumn{2}{l}{Lasso}&\multicolumn{2}{l}{Ridge}&\multicolumn{2}{l}{ElasticNet}&\multicolumn{2}{l}{PCLR}&\multicolumn{2}{l}{LAELR}&\multicolumn{2}{l}{Dropout}&\multicolumn{2}{l}{\LRnn{}}\\
  \textbf{Summary}\\
\sumNegOarCoef{}&-0.53&$^{(-2.64, -0.47)}$&0.00&$^{(-1.26, 0.00)}$&0.00&$^{(-0.68, 0.00)}$&0.00&$^{(-0.92, 0.00)}$&0.00&$^{(-2.36, 0.00)}$&0.00&$^{(-1.71, 0.00)}$&0.00&$^{(-0.40, 0.00)}$&0.00&$^{(0.00, 0.00)}$\\
\sumPosOarCoef{}&3.32&$^{(3.32, 5.99)}$&2.35&$^{(1.96, 3.89)}$&2.32&$^{(1.80, 4.27)}$&2.24&$^{(1.82, 3.89)}$&2.95&$^{(2.30, 5.74)}$&2.55&$^{(2.33, 5.47)}$&2.65&$^{(1.85, 4.08)}$&2.86&$^{(2.56, 4.70)}$\\
\percNegOarCoef{}&0.30&$^{(0.20, 0.60)}$&0.00&$^{(0.00, 0.40)}$&0.00&$^{(0.00, 0.40)}$&0.00&$^{(0.00, 0.40)}$&0.00&$^{(0.00, 0.60)}$&0.00&$^{(0.00, 0.60)}$&0.00&$^{(0.00, 0.30)}$&0.00&$^{(0.00, 0.00)}$\\
\percPosOarCoef{}&0.50&$^{(0.40, 0.80)}$&0.70&$^{(0.50, 0.90)}$&1.00&$^{(0.60, 1.00)}$&0.80&$^{(0.50, 1.00)}$&1.00&$^{(0.40, 1.00)}$&1.00&$^{(0.40, 1.00)}$&1.00&$^{(0.60, 1.00)}$&0.60&$^{(0.40, 0.90)}$\\\EndTableHeader\\\grayline
 \textbf{Complete}\\
Intercept&-2.97&$^{(-4.26, -2.76)}$&-2.70&$^{(-3.54, -2.34)}$&-2.74&$^{(-3.48, -2.49)}$&-2.67&$^{(-3.50, -2.34)}$&-3.15&$^{(-4.10, -2.74)}$&-2.95&$^{(-4.13, -2.72)}$&-2.89&$^{(-3.74, -2.62)}$&-3.00&$^{(-4.35, -2.71)}$\\
Age&0.02&$^{(-0.15, 0.18)}$&-0.01&$^{(-0.10, 0.07)}$&0.01&$^{(-0.12, 0.13)}$&-0.01&$^{(-0.12, 0.12)}$&0.05&$^{(-0.13, 0.28)}$&0.05&$^{(-0.13, 0.28)}$&0.02&$^{(-0.15, 0.15)}$&0.03&$^{(-0.15, 0.19)}$\\
Dys.BSL.1&0.17&$^{(-0.05, 0.43)}$&0.16&$^{(0.01, 0.33)}$&0.21&$^{(0.04, 0.39)}$&0.17&$^{(0.03, 0.39)}$&0.23&$^{(-0.02, 0.44)}$&0.24&$^{(-0.02, 0.46)}$&0.17&$^{(0.04, 0.37)}$&0.18&$^{(-0.03, 0.39)}$\\
Dys.BSL.2&0.34&$^{(0.17, 0.58)}$&0.33&$^{(0.18, 0.57)}$&0.37&$^{(0.21, 0.56)}$&0.35&$^{(0.20, 0.57)}$&0.41&$^{(0.17, 0.65)}$&0.42&$^{(0.18, 0.65)}$&0.32&$^{(0.17, 0.55)}$&0.35&$^{(0.20, 0.60)}$\\
\grayline
Subm.L.Dm&0.10&$^{(-1.16, 0.96)}$&-0.00&$^{(-0.02, 0.48)}$&0.17&$^{(-0.37, 0.53)}$&0.02&$^{(-0.33, 0.45)}$&0.48&$^{(-0.80, 0.96)}$&0.30&$^{(-1.06, 0.71)}$&0.24&$^{(-0.40, 0.55)}$&0.06&$^{(0.00, 1.09)}$\\
Subm.R.Dm&-0.26&$^{(-1.08, 1.56)}$&-0.00&$^{(-0.50, 0.72)}$&0.16&$^{(-0.30, 0.66)}$&0.00&$^{(-0.36, 0.64)}$&0.57&$^{(-0.92, 1.53)}$&0.30&$^{(-0.67, 0.80)}$&0.14&$^{(-0.14, 0.85)}$&0.00&$^{(0.00, 1.37)}$\\
Parotid.L.Dm&-0.05&$^{(-0.34, 0.58)}$&0.01&$^{(-0.15, 0.35)}$&0.11&$^{(-0.20, 0.34)}$&0.04&$^{(-0.17, 0.35)}$&0.04&$^{(-0.37, 0.52)}$&0.28&$^{(-0.31, 0.55)}$&0.09&$^{(-0.16, 0.34)}$&0.00&$^{(0.00, 0.39)}$\\
Parotid.R.Dm&0.21&$^{(-0.44, 0.64)}$&0.15&$^{(-0.00, 0.43)}$&0.22&$^{(0.00, 0.42)}$&0.17&$^{(-0.00, 0.44)}$&0.23&$^{(-0.18, 0.56)}$&0.30&$^{(-0.08, 0.40)}$&0.19&$^{(-0.09, 0.42)}$&0.14&$^{(0.00, 0.43)}$\\
PCM.Sup.Dm&-0.23&$^{(-1.07, 1.74)}$&0.03&$^{(-0.53, 1.24)}$&0.27&$^{(-0.13, 0.74)}$&0.02&$^{(-0.29, 0.84)}$&0.38&$^{(-0.91, 1.38)}$&0.27&$^{(-0.71, 1.24)}$&0.33&$^{(-0.02, 0.97)}$&0.00&$^{(0.00, 1.75)}$\\
PCM.Med.Dm&0.85&$^{(-0.31, 2.40)}$&0.42&$^{(0.01, 1.09)}$&0.28&$^{(0.13, 0.94)}$&0.41&$^{(0.01, 1.15)}$&0.48&$^{(-0.54, 1.39)}$&0.34&$^{(-0.08, 1.62)}$&0.35&$^{(0.11, 0.84)}$&0.65&$^{(0.00, 1.23)}$\\
PCM.Inf.Dm&0.56&$^{(-0.08, 1.61)}$&0.43&$^{(0.01, 0.63)}$&0.27&$^{(0.06, 0.58)}$&0.37&$^{(0.03, 0.63)}$&0.26&$^{(0.00, 1.09)}$&0.15&$^{(0.01, 1.09)}$&0.31&$^{(0.04, 0.54)}$&0.56&$^{(0.00, 0.75)}$\\
Supraglottic.Dm&0.01&$^{(-0.71, 0.70)}$&0.12&$^{(-0.00, 0.59)}$&0.21&$^{(-0.12, 0.46)}$&0.14&$^{(-0.00, 0.42)}$&0.06&$^{(-0.45, 0.67)}$&0.27&$^{(-0.48, 0.54)}$&0.16&$^{(-0.14, 0.47)}$&0.04&$^{(0.00, 0.58)}$\\
OralCavity.Ext.Dm&1.59&$^{(0.59, 2.41)}$&1.19&$^{(0.57, 1.83)}$&0.60&$^{(0.29, 1.47)}$&1.08&$^{(0.35, 1.66)}$&0.37&$^{(0.26, 2.04)}$&0.31&$^{(0.25, 2.25)}$&0.76&$^{(0.32, 1.37)}$&1.41&$^{(0.56, 1.94)}$\\
GlotticArea.Dm&-0.00&$^{(-0.73, 0.79)}$&0.00&$^{(-0.17, 0.37)}$&0.03&$^{(-0.26, 0.46)}$&0.00&$^{(-0.23, 0.40)}$&0.09&$^{(-0.41, 0.43)}$&0.03&$^{(-0.32, 0.67)}$&0.08&$^{(-0.14, 0.32)}$&0.00&$^{(0.00, 0.65)}$\\
\bottomrule
\end{tabular}}
\end{table}

\newpage
\clearpage

\begin{table}[h!]
    \caption{\label{tab:coef:dysext}Model coefficients for \dysextended}
\resizebox{\textwidth}{!}{
\begin{tabular}{lRlRlRlRlRlRlRlRlRlRlRlRlRlRlRlRlR}\toprule 
 &\multicolumn{2}{l}{LR}&\multicolumn{2}{l}{Lasso}&\multicolumn{2}{l}{Ridge}&\multicolumn{2}{l}{ElasticNet}&\multicolumn{2}{l}{PCLR}&\multicolumn{2}{l}{LAELR}&\multicolumn{2}{l}{Dropout}&\multicolumn{2}{l}{\LRnn{}}\\
  \textbf{Summary}\\
\sumNegOarCoef{}&-8.54&$^{(-18.39, -8.54)}$&-0.04&$^{(-5.26, 0.00)}$&-0.22&$^{(-10.59, -0.01)}$&-0.10&$^{(-4.95, 0.00)}$&-0.82&$^{(-39.06, -0.14)}$&-1.77&$^{(-26.01, 0.00)}$&-0.48&$^{(-3.40, -0.19)}$&0.00&$^{(0.00, 0.00)}$\\
\sumPosOarCoef{}&12.69&$^{(12.69, 24.08)}$&2.11&$^{(1.76, 10.17)}$&2.60&$^{(2.30, 15.81)}$&2.22&$^{(2.09, 8.27)}$&5.05&$^{(2.36, 45.09)}$&5.85&$^{(2.34, 34.12)}$&3.36&$^{(2.93, 7.06)}$&4.83&$^{(3.64, 6.79)}$\\
\percNegOarCoef{}&0.47&$^{(0.38, 0.57)}$&0.07&$^{(0.00, 0.28)}$&0.10&$^{(0.03, 0.50)}$&0.07&$^{(0.00, 0.40)}$&0.28&$^{(0.10, 0.50)}$&0.33&$^{(0.00, 0.53)}$&0.15&$^{(0.05, 0.42)}$&0.00&$^{(0.00, 0.00)}$\\
\percPosOarCoef{}&0.53&$^{(0.40, 0.62)}$&0.25&$^{(0.23, 0.47)}$&0.85&$^{(0.50, 0.90)}$&0.68&$^{(0.23, 0.85)}$&0.68&$^{(0.50, 0.88)}$&0.65&$^{(0.47, 0.97)}$&0.80&$^{(0.55, 0.85)}$&0.28&$^{(0.20, 0.40)}$\\\EndTableHeader\\\grayline
 \textbf{Complete}\\
Intercept&-3.44&$^{(-4.24, -3.42)}$&-2.53&$^{(-3.85, -2.30)}$&-2.65&$^{(-3.96, -2.46)}$&-2.56&$^{(-3.58, -2.33)}$&-3.07&$^{(-5.07, -2.63)}$&-3.24&$^{(-4.85, -2.59)}$&-2.79&$^{(-3.55, -2.68)}$&-3.38&$^{(-4.25, -3.25)}$\\
Age&0.08&$^{(-0.11, 0.28)}$&-0.00&$^{(-0.09, 0.18)}$&0.01&$^{(-0.11, 0.21)}$&0.00&$^{(-0.10, 0.22)}$&0.04&$^{(-0.10, 0.20)}$&0.04&$^{(-0.21, 0.27)}$&-0.00&$^{(-0.14, 0.17)}$&0.04&$^{(-0.13, 0.21)}$\\
Dys.BSL.1&0.16&$^{(-0.02, 0.46)}$&0.15&$^{(0.00, 0.32)}$&0.16&$^{(0.03, 0.31)}$&0.16&$^{(0.01, 0.34)}$&0.20&$^{(-0.01, 0.42)}$&0.18&$^{(-0.11, 0.37)}$&0.09&$^{(-0.01, 0.29)}$&0.18&$^{(-0.01, 0.37)}$\\
Dys.BSL.1&0.34&$^{(0.13, 0.77)}$&0.32&$^{(0.17, 0.57)}$&0.32&$^{(0.18, 0.56)}$&0.31&$^{(0.18, 0.57)}$&0.37&$^{(0.01, 0.67)}$&0.34&$^{(0.03, 0.63)}$&0.21&$^{(0.10, 0.58)}$&0.35&$^{(0.19, 0.61)}$\\
\grayline
Subm.L.Dm&0.49&$^{(-1.09, 1.87)}$&0.00&$^{(-0.00, 0.68)}$&0.09&$^{(-0.09, 0.64)}$&0.08&$^{(-0.05, 0.48)}$&0.13&$^{(-0.41, 0.53)}$&0.15&$^{(-0.10, 1.85)}$&0.12&$^{(-0.07, 0.35)}$&0.00&$^{(0.00, 0.90)}$\\
Subm.L.V10&-0.19&$^{(-1.55, 1.36)}$&-0.00&$^{(-0.01, 0.01)}$&0.02&$^{(-0.19, 0.30)}$&0.00&$^{(-0.18, 0.29)}$&0.06&$^{(-17.86, 0.90)}$&0.12&$^{(-2.96, 0.40)}$&0.07&$^{(-0.26, 0.27)}$&0.00&$^{(0.00, 1.07)}$\\
Subm.L.V30&0.07&$^{(-1.65, 2.15)}$&0.00&$^{(-0.01, 0.95)}$&0.02&$^{(-0.82, 0.96)}$&0.00&$^{(-0.10, 0.69)}$&0.01&$^{(-0.59, 21.70)}$&0.05&$^{(-1.72, 5.45)}$&-0.02&$^{(-0.64, 0.48)}$&0.00&$^{(0.00, 1.75)}$\\
Subm.L.V50&-0.48&$^{(-1.33, 0.61)}$&0.00&$^{(-0.39, 0.16)}$&0.04&$^{(-0.43, 0.14)}$&0.04&$^{(-0.58, 0.14)}$&0.19&$^{(-0.59, 0.36)}$&0.06&$^{(-1.50, 0.16)}$&0.02&$^{(-0.48, 0.17)}$&0.00&$^{(0.00, 0.03)}$\\
\grayline
Subm.R.Dm&-0.46&$^{(-1.51, 1.91)}$&0.01&$^{(-0.08, 0.56)}$&0.07&$^{(-0.17, 0.30)}$&0.06&$^{(-0.21, 0.63)}$&0.02&$^{(-0.43, 1.08)}$&0.05&$^{(-0.73, 0.94)}$&0.12&$^{(-0.10, 0.48)}$&0.00&$^{(0.00, 1.09)}$\\
Subm.R.V10&-0.04&$^{(-0.83, 1.07)}$&0.00&$^{(-0.00, 0.01)}$&0.01&$^{(-0.05, 0.26)}$&0.00&$^{(-0.00, 0.24)}$&-0.02&$^{(-1.87, 0.55)}$&0.09&$^{(-0.71, 1.19)}$&0.08&$^{(-0.18, 0.27)}$&0.00&$^{(0.00, 0.00)}$\\
Subm.R.V30&-0.27&$^{(-2.22, 2.39)}$&0.00&$^{(-0.89, 0.01)}$&-0.00&$^{(-0.72, 0.36)}$&0.00&$^{(-0.46, 0.25)}$&-0.08&$^{(-1.60, 1.18)}$&-0.01&$^{(-2.33, 2.24)}$&-0.14&$^{(-0.47, 0.18)}$&0.00&$^{(0.00, 0.40)}$\\
Subm.R.V50&0.30&$^{(-1.13, 1.57)}$&0.01&$^{(-0.16, 0.45)}$&0.06&$^{(-0.62, 0.60)}$&0.05&$^{(-0.65, 0.42)}$&0.00&$^{(-0.72, 1.40)}$&-0.11&$^{(-0.64, 0.58)}$&0.05&$^{(-0.45, 0.40)}$&0.00&$^{(0.00, 0.45)}$\\
\grayline
Parotid.L.Dm&0.04&$^{(-2.05, 2.42)}$&0.00&$^{(-0.02, 0.25)}$&0.03&$^{(-0.62, 0.25)}$&0.03&$^{(-0.02, 0.25)}$&-0.03&$^{(-0.87, 0.11)}$&-0.05&$^{(-2.96, 0.14)}$&0.01&$^{(-0.21, 0.14)}$&0.00&$^{(0.00, 0.28)}$\\
Parotid.L.V10&0.43&$^{(-0.95, 1.36)}$&0.05&$^{(-0.09, 0.30)}$&0.09&$^{(-0.23, 0.71)}$&0.08&$^{(-0.22, 0.54)}$&-0.03&$^{(-0.27, 0.89)}$&-0.03&$^{(-0.49, 1.14)}$&0.06&$^{(-0.09, 0.34)}$&0.02&$^{(0.00, 0.14)}$\\
Parotid.L.V30&-0.02&$^{(-1.57, 1.17)}$&0.00&$^{(-0.22, 0.27)}$&0.00&$^{(-0.55, 0.24)}$&0.00&$^{(-0.55, 0.23)}$&-0.05&$^{(-0.31, 0.31)}$&0.06&$^{(-0.09, 1.19)}$&0.03&$^{(-0.30, 0.11)}$&0.00&$^{(0.00, 0.23)}$\\
Parotid.L.V50&-0.12&$^{(-0.95, 0.88)}$&0.00&$^{(-0.27, 0.19)}$&0.01&$^{(-0.36, 0.18)}$&0.01&$^{(-0.26, 0.21)}$&0.01&$^{(-0.28, 0.36)}$&-0.05&$^{(-0.46, 0.93)}$&-0.00&$^{(-0.24, 0.14)}$&0.00&$^{(0.00, 0.21)}$\\
\grayline
Parotid.R.Dm&1.01&$^{(-0.58, 3.07)}$&0.01&$^{(-0.00, 0.22)}$&0.06&$^{(-0.00, 0.88)}$&0.06&$^{(-0.00, 0.43)}$&0.02&$^{(-0.77, 0.18)}$&0.07&$^{(-0.31, 6.45)}$&0.09&$^{(-0.07, 0.26)}$&0.00&$^{(0.00, 0.20)}$\\
Parotid.R.V10&-0.29&$^{(-1.55, 0.53)}$&0.00&$^{(-0.34, 0.22)}$&0.03&$^{(-0.73, 0.15)}$&0.02&$^{(-0.35, 0.11)}$&-0.13&$^{(-0.64, 0.28)}$&-0.09&$^{(-2.40, 0.27)}$&0.02&$^{(-0.18, 0.24)}$&0.00&$^{(0.00, 0.26)}$\\
Parotid.R.V30&-0.58&$^{(-2.09, 0.50)}$&-0.00&$^{(-0.05, 0.12)}$&0.02&$^{(-0.46, 0.10)}$&0.02&$^{(-0.16, 0.12)}$&0.03&$^{(-0.43, 0.40)}$&0.13&$^{(-2.22, 0.45)}$&0.05&$^{(-0.19, 0.19)}$&0.00&$^{(0.00, 0.16)}$\\
Parotid.R.V50&-0.04&$^{(-1.14, 1.29)}$&0.09&$^{(-0.03, 0.30)}$&0.08&$^{(-0.17, 0.46)}$&0.08&$^{(-0.18, 0.44)}$&0.14&$^{(-0.32, 0.61)}$&0.00&$^{(-2.39, 0.39)}$&0.06&$^{(-0.11, 0.29)}$&0.10&$^{(0.00, 0.32)}$\\
\grayline
PCM.Sup.Dm&0.54&$^{(-0.93, 2.47)}$&0.00&$^{(-0.04, 0.29)}$&0.08&$^{(-0.19, 0.58)}$&0.08&$^{(-0.19, 0.35)}$&0.11&$^{(-1.18, 0.32)}$&0.09&$^{(-1.33, 1.02)}$&0.11&$^{(-0.16, 0.36)}$&0.00&$^{(0.00, 1.16)}$\\
PCM.Sup.V10&-1.49&$^{(-4.32, 0.33)}$&0.00&$^{(-0.96, 0.02)}$&-0.02&$^{(-0.64, 0.03)}$&0.00&$^{(-0.86, 0.01)}$&-0.03&$^{(-1.68, 0.21)}$&-0.25&$^{(-2.24, 0.17)}$&-0.10&$^{(-0.83, 0.08)}$&0.00&$^{(0.00, 0.00)}$\\
PCM.Sup.V30&-0.43&$^{(-2.59, 1.24)}$&0.01&$^{(-1.14, 0.01)}$&0.03&$^{(-1.37, 0.30)}$&0.02&$^{(-0.84, 0.10)}$&0.04&$^{(-1.61, 0.83)}$&-0.09&$^{(-1.88, 1.03)}$&0.06&$^{(-0.50, 0.28)}$&0.00&$^{(0.00, 0.00)}$\\
PCM.Sup.V50&-0.22&$^{(-1.30, 0.64)}$&0.00&$^{(-0.23, 0.69)}$&0.12&$^{(-0.26, 0.40)}$&0.12&$^{(-0.26, 0.44)}$&0.21&$^{(-0.38, 0.80)}$&0.29&$^{(-0.46, 0.55)}$&0.12&$^{(-0.16, 0.34)}$&0.00&$^{(0.00, 0.47)}$\\
\grayline
PCM.Med.Dm&0.68&$^{(-1.52, 2.95)}$&0.52&$^{(-0.00, 1.50)}$&0.15&$^{(-0.51, 0.75)}$&0.14&$^{(-0.00, 1.02)}$&0.04&$^{(-0.26, 1.80)}$&0.31&$^{(-1.11, 2.34)}$&0.17&$^{(-0.03, 0.69)}$&0.59&$^{(0.00, 1.06)}$\\
PCM.Med.V10&1.01&$^{(-2.15, 2.18)}$&0.00&$^{(-0.01, 0.01)}$&0.06&$^{(-0.37, 0.72)}$&0.03&$^{(-0.00, 0.50)}$&0.20&$^{(-5.57, 3.74)}$&0.56&$^{(-6.92, 2.28)}$&0.14&$^{(-0.04, 0.65)}$&1.15&$^{(0.00, 1.69)}$\\
PCM.Med.V30&1.37&$^{(-0.69, 3.84)}$&0.00&$^{(0.00, 2.25)}$&0.08&$^{(0.01, 2.26)}$&0.05&$^{(-0.00, 1.40)}$&-0.01&$^{(-0.43, 4.49)}$&0.34&$^{(-0.50, 4.57)}$&0.16&$^{(-0.03, 0.79)}$&0.00&$^{(0.00, 2.11)}$\\
PCM.Med.V50&-0.54&$^{(-1.35, 0.50)}$&-0.01&$^{(-0.58, 0.09)}$&0.03&$^{(-0.35, 0.13)}$&0.03&$^{(-0.50, 0.14)}$&-0.11&$^{(-1.03, 0.46)}$&-0.10&$^{(-1.21, 0.56)}$&0.04&$^{(-0.24, 0.12)}$&0.00&$^{(0.00, 0.04)}$\\
\grayline
PCM.Inf.Dm&2.24&$^{(0.39, 4.24)}$&0.35&$^{(0.01, 2.20)}$&0.17&$^{(0.05, 2.10)}$&0.16&$^{(0.03, 1.23)}$&0.18&$^{(-0.00, 4.27)}$&0.39&$^{(0.02, 4.02)}$&0.05&$^{(0.05, 0.56)}$&0.39&$^{(0.00, 0.74)}$\\
PCM.Inf.V10&0.32&$^{(-0.93, 1.07)}$&-0.02&$^{(-0.02, 0.02)}$&0.03&$^{(-0.13, 0.17)}$&0.01&$^{(-0.01, 0.05)}$&0.57&$^{(-3.26, 1.87)}$&0.27&$^{(-0.76, 1.96)}$&0.23&$^{(-0.03, 0.91)}$&0.82&$^{(0.00, 1.42)}$\\
PCM.Inf.V30&-0.76&$^{(-1.37, -0.00)}$&-0.01&$^{(-0.69, 0.01)}$&-0.07&$^{(-0.57, 0.06)}$&-0.04&$^{(-0.56, 0.07)}$&-0.04&$^{(-1.34, 0.35)}$&-0.33&$^{(-1.15, 0.32)}$&-0.11&$^{(-0.48, 0.19)}$&0.00&$^{(0.00, 0.00)}$\\
PCM.Inf.V50&-1.10&$^{(-2.70, 0.38)}$&0.00&$^{(-1.17, 0.38)}$&0.07&$^{(-1.04, 0.20)}$&0.06&$^{(-0.67, 0.34)}$&0.28&$^{(-2.73, 0.47)}$&0.11&$^{(-2.57, 0.52)}$&0.11&$^{(-0.20, 0.28)}$&0.00&$^{(0.00, 0.41)}$\\
\grayline
Supraglottic.Dm&0.36&$^{(-1.87, 2.29)}$&0.03&$^{(-0.36, 0.98)}$&0.14&$^{(-0.58, 1.50)}$&0.13&$^{(-0.00, 0.90)}$&0.18&$^{(-1.74, 1.81)}$&0.36&$^{(-2.10, 1.91)}$&0.10&$^{(-0.09, 0.47)}$&0.00&$^{(0.00, 0.34)}$\\
Supraglottic.V10&-0.21&$^{(-1.97, 0.92)}$&-0.00&$^{(-0.00, 0.02)}$&0.03&$^{(-0.23, 0.31)}$&0.00&$^{(-0.00, 0.10)}$&0.61&$^{(-3.30, 2.71)}$&0.61&$^{(-0.60, 2.64)}$&0.06&$^{(-0.09, 0.51)}$&0.00&$^{(0.00, 0.00)}$\\
Supraglottic.V30&-0.50&$^{(-1.38, 0.74)}$&0.00&$^{(-0.78, 0.01)}$&-0.06&$^{(-1.00, 0.26)}$&-0.01&$^{(-0.73, 0.22)}$&0.03&$^{(-1.36, 0.65)}$&0.02&$^{(-1.37, 0.48)}$&-0.09&$^{(-0.51, 0.26)}$&0.00&$^{(0.00, 0.00)}$\\
Supraglottic.V50&0.24&$^{(-0.97, 1.54)}$&0.08&$^{(-0.02, 0.61)}$&0.11&$^{(-0.42, 0.39)}$&0.11&$^{(-0.35, 0.27)}$&0.20&$^{(-0.88, 1.51)}$&-0.12&$^{(-1.11, 1.61)}$&0.12&$^{(-0.35, 0.28)}$&0.02&$^{(0.00, 0.20)}$\\
\grayline
OralCavity.Ext.Dm&0.69&$^{(-1.18, 1.72)}$&0.01&$^{(0.00, 0.60)}$&0.20&$^{(-0.08, 1.02)}$&0.19&$^{(-0.00, 0.52)}$&0.31&$^{(0.08, 0.66)}$&0.23&$^{(-1.41, 0.91)}$&0.20&$^{(0.05, 0.73)}$&0.00&$^{(0.00, 1.16)}$\\
OralCavity.Ext.V10&0.48&$^{(-1.24, 1.59)}$&0.01&$^{(-0.61, 0.01)}$&0.02&$^{(-0.96, 0.26)}$&0.00&$^{(-0.44, 0.33)}$&0.03&$^{(-1.43, 0.55)}$&-0.24&$^{(-1.34, 2.09)}$&0.01&$^{(-0.43, 0.24)}$&0.00&$^{(0.00, 0.06)}$\\
OralCavity.Ext.V30&0.43&$^{(-0.44, 2.45)}$&0.28&$^{(0.00, 1.20)}$&0.16&$^{(0.10, 1.20)}$&0.15&$^{(0.08, 0.90)}$&0.27&$^{(0.05, 1.66)}$&0.14&$^{(0.05, 1.79)}$&0.21&$^{(0.08, 0.59)}$&0.48&$^{(0.00, 1.49)}$\\
OralCavity.Ext.V50&0.55&$^{(-0.03, 1.39)}$&0.63&$^{(0.23, 1.15)}$&0.31&$^{(0.18, 0.90)}$&0.30&$^{(0.18, 1.08)}$&0.48&$^{(0.01, 1.26)}$&0.74&$^{(0.04, 1.38)}$&0.24&$^{(0.12, 0.67)}$&0.72&$^{(0.00, 1.03)}$\\
\grayline
GlotticArea.Dm&-0.80&$^{(-2.44, 1.23)}$&0.01&$^{(-0.93, 0.03)}$&0.05&$^{(-1.45, 0.15)}$&0.02&$^{(-0.66, 0.12)}$&-0.00&$^{(-2.11, 1.16)}$&0.33&$^{(-1.88, 0.68)}$&0.06&$^{(-0.04, 0.21)}$&0.00&$^{(0.00, 0.41)}$\\
GlotticArea.V10&0.73&$^{(-0.90, 2.66)}$&0.00&$^{(-0.01, 0.02)}$&0.02&$^{(0.01, 0.78)}$&0.00&$^{(-0.01, 0.06)}$&0.53&$^{(-0.17, 2.85)}$&0.20&$^{(-1.60, 3.74)}$&0.24&$^{(-0.06, 0.68)}$&0.29&$^{(0.00, 1.85)}$\\
GlotticArea.V30&0.17&$^{(-1.03, 1.45)}$&-0.02&$^{(-0.57, 0.32)}$&-0.07&$^{(-0.80, 0.29)}$&-0.05&$^{(-0.73, 0.36)}$&-0.29&$^{(-1.46, 0.35)}$&-0.32&$^{(-1.45, 0.72)}$&-0.03&$^{(-0.72, 0.31)}$&0.00&$^{(0.00, 0.52)}$\\
GlotticArea.V50&0.52&$^{(-0.64, 1.96)}$&0.07&$^{(-0.00, 1.04)}$&0.10&$^{(-0.11, 1.36)}$&0.09&$^{(-0.08, 0.83)}$&0.16&$^{(-0.41, 1.75)}$&0.08&$^{(-0.32, 1.74)}$&0.14&$^{(-0.11, 0.45)}$&0.25&$^{(0.00, 0.86)}$\\
\bottomrule
\end{tabular}}
\end{table}

==> sections/3-TABS-PERF.tex <==


\begin{table}[h!]
    \centering
    \caption{\label{tab:res:perf}Results from (1) internal validation, and (2), external validation. *It is important to notice that the external validation data is quite small (only 25 events for xerostomia, and 9 for dysphagia), resulting in large confidence intervals.}
    \resizebox{.8\textwidth}{!}{
    \begin{tabular}{lcccccccccccccccc}
    \toprule
    &\multicolumn{3}{c}{\textbf{Internal}}&&\multicolumn{3}{c}{\textbf{External}*}\\
    \cmidrule{2-4}\cmidrule{6-8}
\textbf{Model}&\auroc&\citl&\cslope && \auroc&\citl&\cslope\\
\midrule
\hspace{-.2cm}\xerbasic\\
LR&0.77$^{(0.77, 0.78)}$&0.00$^{(-0.00, 0.02)}$&0.86$^{(0.75, 0.96)}$ &&0.75$^{(0.59, 0.83)}$&-0.55$^{(-1.00, 0.03)}$&0.65$^{(0.20, 0.97)}$\\
Lasso&0.78$^{(0.77, 0.79)}$&-0.00$^{(-0.01, 0.01)}$&1.03$^{(1.03, 1.20)}$&&0.76$^{(0.59, 0.84)}$&-0.50$^{(-0.94, 0.01)}$&0.94$^{(0.24, 1.28)}$\\
Ridge&0.77$^{(0.77, 0.79)}$&-0.01$^{(-0.01, 0.01)}$&1.00$^{(1.00, 1.23)}$&&0.77$^{(0.60, 0.86)}$&-0.56$^{(-0.95, -0.04)}$&0.90$^{(0.25, 1.38)}$\\
ElasticNet&0.78$^{(0.78, 0.79)}$&-0.01$^{(-0.01, 0.01)}$&0.99$^{(0.99, 1.22)}$&&0.77$^{(0.59, 0.84)}$&-0.52$^{(-0.94, -0.03)}$&0.94$^{(0.26, 1.23)}$\\
PCLR&0.77$^{(0.77, 0.78)}$&-0.02$^{(-0.02, 0.02)}$&0.79$^{(0.76, 0.97)}$&&0.77$^{(0.59, 0.87)}$&-0.53$^{(-0.97, 0.00)}$&0.69$^{(0.20, 1.35)}$\\
LAELR&0.78$^{(0.77, 0.78)}$&-0.01$^{(-0.01, 0.03)}$&0.91$^{(0.75, 0.96)}$&&0.76$^{(0.59, 0.87)}$&-0.53$^{(-0.98, 0.01)}$&0.69$^{(0.20, 1.35)}$\\
Dropout&0.77$^{(0.77, 0.79)}$&0.02$^{(0.01, 0.05)}$&0.93$^{(0.93, 1.34)}$&&0.77$^{(0.59, 0.86)}$&-0.51$^{(-0.88, -0.04)}$&1.04$^{(0.20, 2.26)}$\\
\LRnn{}&0.77$^{(0.77, 0.79)}$&0.00$^{(-0.01, 0.02)}$&0.86$^{(0.81, 0.97)}$&&0.75$^{(0.58, 0.83)}$&-0.54$^{(-1.00, 0.03)}$&0.65$^{(0.18, 1.08)}$\\
\grayline
\hspace{-.2cm} \xerextended\\
LR&0.75$^{(0.75, 0.78)}$&-0.04$^{(-0.04, 0.02)}$&0.67$^{(0.63, 0.83)}$&&0.77$^{(0.61, 0.87)}$&-0.61$^{(-1.06, -0.04)}$&0.58$^{(0.15, 0.92)}$\\
Lasso&0.77$^{(0.77, 0.78)}$&-0.01$^{(-0.01, 0.01)}$&1.05$^{(1.05, 1.19)}$&&0.78$^{(0.63, 0.87)}$&-0.51$^{(-0.87, -0.02)}$&0.94$^{(0.35, 1.37)}$\\
Ridge&0.78$^{(0.78, 0.78)}$&-0.01$^{(-0.01, 0.01)}$&1.05$^{(1.05, 1.21)}$&&0.78$^{(0.62, 0.86)}$&-0.47$^{(-0.87, 0.01)}$&0.95$^{(0.27, 1.35)}$\\
ElasticNet&0.77$^{(0.77, 0.78)}$&-0.01$^{(-0.01, 0.01)}$&1.04$^{(1.04, 1.22)}$&&0.78$^{(0.62, 0.87)}$&-0.48$^{(-0.87, -0.00)}$&0.92$^{(0.32, 1.41)}$\\
PCLR&0.77$^{(0.77, 0.78)}$&0.01$^{(-0.03, 0.01)}$&0.84$^{(0.72, 1.00)}$&&0.75$^{(0.24, 0.85)}$&-0.27$^{(-1.41, 0.17)}$&0.63$^{(-0.00, 1.17)}$\\
LAELR&0.77$^{(0.77, 0.79)}$&0.01$^{(-0.03, 0.03)}$&0.63$^{(0.63, 1.01)}$&&0.75$^{(0.60, 0.86)}$&-0.27$^{(-1.20, 0.18)}$&0.64$^{(0.15, 0.94)}$\\
Dropout&0.77$^{(0.77, 0.79)}$&-0.01$^{(-0.01, 0.05)}$&0.88$^{(0.82, 1.17)}$&&0.77$^{(0.62, 0.88)}$&-0.50$^{(-0.89, 0.08)}$&0.82$^{(0.12, 1.92)}$\\
\LRnn{}&0.77$^{(0.77, 0.78)}$&-0.01$^{(-0.01, 0.03)}$&0.78$^{(0.68, 0.88)}$&&0.77$^{(0.62, 0.85)}$&-0.57$^{(-1.01, 0.01)}$&0.59$^{(0.12, 0.86)}$\\
\grayline
\hspace{-.2cm} \dysbasic\\
LR&0.83$^{(0.82, 0.84)}$&-0.01$^{(-0.03, 0.02)}$&0.82$^{(0.75, 0.88)}$&&0.92$^{(0.83, 0.97)}$&-0.56$^{(-1.58, 0.26)}$&1.18$^{(0.78, 1.84)}$\\
Lasso&0.85$^{(0.83, 0.85)}$&-0.03$^{(-0.03, 0.01)}$&1.04$^{(0.97, 1.11)}$&&0.91$^{(0.87, 0.97)}$&-0.60$^{(-1.57, 0.25)}$&1.35$^{(0.94, 2.23)}$\\
Ridge&0.84$^{(0.83, 0.84)}$&-0.01$^{(-0.02, 0.02)}$&1.08$^{(0.97, 1.09)}$&&0.91$^{(0.87, 0.97)}$&-0.64$^{(-1.66, 0.18)}$&1.39$^{(1.01, 2.42)}$\\
ElasticNet&0.84$^{(0.83, 0.85)}$&-0.00$^{(-0.02, 0.02)}$&1.11$^{(0.96, 1.11)}$&&0.91$^{(0.87, 0.98)}$&-0.60$^{(-1.61, 0.21)}$&1.37$^{(1.01, 2.24)}$\\
PCLR&0.84$^{(0.82, 0.84)}$&-0.00$^{(-0.02, 0.06)}$&0.87$^{(0.78, 0.95)}$&&0.91$^{(0.86, 0.97)}$&-0.66$^{(-1.78, 0.12)}$&1.26$^{(0.86, 2.87)}$\\
LAELR&0.84$^{(0.82, 0.84)}$&-0.03$^{(-0.03, 0.05)}$&0.90$^{(0.80, 0.95)}$&&0.90$^{(0.85, 0.97)}$&-0.61$^{(-1.61, 0.18)}$&1.21$^{(0.86, 3.37)}$\\
Dropout&0.84$^{(0.83, 0.84)}$&0.02$^{(-0.00, 0.09)}$&1.12$^{(0.96, 1.16)}$&&0.92$^{(0.87, 0.98)}$&-0.58$^{(-1.63, 0.27)}$&1.37$^{(1.01, 2.81)}$\\
\LRnn{}&0.84$^{(0.83, 0.84)}$&-0.02$^{(-0.03, 0.01)}$&0.88$^{(0.80, 0.92)}$&&0.92$^{(0.86, 0.97)}$&-0.57$^{(-1.58, 0.33)}$&1.19$^{(0.81, 2.23)}$\\
\grayline
\hspace{-.2cm} \dysextended\\
LR&0.80$^{(0.79, 0.82)}$&-0.04$^{(-0.08, 0.00)}$&0.59$^{(0.54, 0.66)}$&&0.86$^{(0.75, 0.95)}$&-0.64$^{(-2.35, 0.51)}$&0.85$^{(0.39, 1.39)}$\\
Lasso&0.84$^{(0.83, 0.84)}$&-0.01$^{(-0.02, 0.02)}$&1.09$^{(0.98, 1.12)}$&&0.90$^{(0.82, 0.96)}$&-0.68$^{(-1.71, 0.15)}$&1.42$^{(0.58, 2.43)}$\\
Ridge&0.84$^{(0.83, 0.84)}$&-0.01$^{(-0.02, 0.02)}$&1.11$^{(0.99, 1.14)}$&&0.91$^{(0.83, 0.96)}$&-0.54$^{(-1.86, 0.29)}$&1.42$^{(0.49, 3.58)}$\\
ElasticNet&0.84$^{(0.83, 0.84)}$&-0.01$^{(-0.02, 0.02)}$&1.12$^{(0.96, 1.13)}$&&0.91$^{(0.83, 0.97)}$&-0.58$^{(-1.65, 0.27)}$&1.48$^{(0.66, 2.69)}$\\
PCLR&0.83$^{(0.81, 0.84)}$&-0.08$^{(-0.08, 0.03)}$&0.85$^{(0.72, 0.91)}$&&0.90$^{(0.80, 0.96)}$&-0.54$^{(-1.99, 0.49)}$&1.14$^{(0.34, 1.89)}$\\
LAELR&0.82$^{(0.80, 0.84)}$&-0.09$^{(-0.09, 0.08)}$&0.85$^{(0.72, 0.91)}$&&0.89$^{(0.79, 0.94)}$&-0.73$^{(-2.50, 0.29)}$&1.22$^{(0.33, 1.88)}$\\
Dropout&0.84$^{(0.82, 0.84)}$&0.03$^{(0.01, 0.14)}$&1.08$^{(0.95, 1.14)}$&&0.92$^{(0.84, 0.97)}$&-0.45$^{(-1.32, 0.35)}$&1.58$^{(0.83, 3.26)}$\\
\LRnn{}&0.84$^{(0.83, 0.84)}$&-0.03$^{(-0.04, 0.01)}$&0.85$^{(0.77, 0.87)}$&&0.90$^{(0.78, 0.97)}$&-0.58$^{(-1.51, 0.37)}$&1.23$^{(0.85, 2.25)}$\\
\bottomrule
    \end{tabular}}
\end{table}



==> sections/BOXPLOTS-REAL.tex <==
\newcommand\boxplotwidth{0.48\textwidth}
\begin{figure}[h!]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=\boxplotwidth]{img/boxplots/CompareMethods-real-A-ExpJacc.pdf}& \includegraphics[width=\boxplotwidth]{img/boxplots/CompareMethods-real-C-ExpJacc.pdf}\\
    \end{tabular}
    \caption{Per method, the mean proportion of coefficients with the same direction of effect after repetition for the \textbf{real-data} settings. Red indicates low collinearity and higher EPV, and blue high collinearity and lower EPV.}
    \label{fig:mijcs_results_real}
\end{figure}
